Token Prediction as Implicit Classification to Identify LLM-Generated Text

This paper introduces a novel approach for identifying the possible large language models (LLMs) involved in text generation. Instead of adding an additional classification layer to a base LM, we reframe the classification task as a next-token prediction task and directly fine-tune the base LM to perform it. We utilize the Text-to-Text Transfer Transformer (T5) model as the backbone for our experiments. We compared our approach to the more direct approach of utilizing hidden states for classification. Evaluation shows the exceptional performance of our method in the text classification task, highlighting its simplicity and efficiency. Furthermore, interpretability studies on the features extracted by our model reveal its ability to differentiate distinctive writing styles among various LLMs even in the absence of an explicit classifier. We also collected a dataset named OpenLLMText, containing approximately 340k text samples from human and LLMs, including GPT3.5, PaLM, LLaMA, and GPT2.

==> content/acknowledgement.tex <==
We would like to express our sincere appreciation to Professor Bhiksha Raj and  Liangze (Josh) Li for their invaluable guidance, insightful comments, and constant support throughout the course of this research. Their expertise in the field have been instrumental in shaping our work.

